CAKE: An Efficient Group Key Management for Dynamic Groups

With rapid increase of mobile computing and wireless network linkage, the information exchange between connected systems and within groups increases heavily. Exchanging confidential information within groups via unsecured communication channels is a high security threat. In order to prevent third parties from accessing this data, it is essential to encrypt it. For this purpose, the group participants need a common group key to enable encrypted broadcast messages. But efficient key management of secured group communication is a challenging task, if participants rely on low performance hardware and small bandwidth. For coordination and distribution, we present the modular group key management procedure CAKE that is centrally organized and meets strict security requirements. The lightweight G-IKEv2 protocol in combination with the key exchange concept of CAKE leads to an efficiently integrated solution. The hybrid approach combines the advantages of the existing protocols with the objective to reduce the computation and communication effort. It is shown that the procedure is more suitable for changing MANET groups than the existing ones. Moreover, the exchanged group key can be used for any services which provides a wide range of applications.

==> abstract.tex <==
\begin{abstract}
With rapid increase of mobile computing and wireless network linkage, the information exchange between connected systems and within groups increases heavily.
Exchanging confidential information within groups via unsecured communication channels is a high security threat.
%In order to prevent third parties from accessing this data, it is essential to encrypt it.
For this purpose, the group participants need a common group key to enable encrypted broadcast messages.
But efficient key management of secured group communication is a challenging task, if participants rely on low performance hardware and small bandwidth.
%Especially, dynamically changing group compositions generate large management overhead.
For coordination and distribution, we present the modular group key management procedure CAKE that is centrally organized and meets strict security requirements.
The lightweight G-IKEv2 protocol in combination with the key exchange concept of CAKE leads to an efficiently integrated solution.
The hybrid approach combines the advantages of the existing protocols with the objective to reduce the computation and communication effort. 
It is shown that the procedure is more suitable for changing MANET groups than the existing ones.
%Moreover, the exchanged group key can be used for any services which provides a wide range of applications.
\end{abstract}


==> picture/plot-data.tex <==





==> picture/table-memory-requirements.tex <==
\newcommand{\riot}[1]{\multicolumn{1}{r@{\,}}{#1} & \multicolumn{1}{@{}l}{Byte}}
\newcommand{\tablebulletpoint}{\quad $\lhookrightarrow$\,}
\newcommand{\tbp}{\tablebulletpoint}
\newcommand{\tbptwo}{\quad \tablebulletpoint}

\begin{table}[t]
  \centering
  \caption{Memory required of the test setup (with 16\,Byte CAKE key size and 17\,Byte CAKE Prime size)\todo[inline]{Tobi: Die Zahlen stimmen noch nicht zu 100\%}}
  \label{tab:memory-requirements}
  \begin{threeparttable}[b]
  \begin{tabular}{l|rr}
    \textbf{Feature}         					   	& \textbf{Server} 					 	& \textbf{Client}			\\
    \hline					                                       						
    RIOT kernel (incl. stack)					   	&	\riot{2,048}																	\\
		RIOT 802.15.4 module cache						& \riot{1,024}																	\\
		RIOT 6LoWPAN cache										& \riot{1,536}																	\\
    RIOT IPv6 stack (incl. net discovery)	& \riot{2,240}																	\\
    RIOT UDP stack           					   	& \riot{1,024}																	\\
    RIOT net cache           					   	& \riot{1,216}																	\\
    RIOT packet buffer       					   	& \riot{2,048}																	\\
		RIOT AES library											& \riot{10,240}																	\\
		RIOT Mini-GMP Library									& \riot{2,574}																	\\
		\hline                                                 											
		$\sum$ RIOT														& \riot{23,950}																	\\
		\hline                                                 					
		\textit{CAKE Tree Keys}   						& 1,024\,Byte\tnote{b}				&  112\,Byte\tnote{c}      \\
		\textit{CAKE Tree Primes}  						& 2,176\,Byte\tnote{d}				&  119\,Byte\tnote{e}      \\
		\textit{CAKE Stack}										& 5,048\,Byte									&  3,464\,Byte	      \\
    \hline                                                 							                    
    $\sum$ CAKE                  					& 8,248\,Byte   							& 3,695\,Byte      \\
		\hline                                           						      	              
		\textit{CAKE SA}											& $\sim$2900\,Byte\tnote{e}   & 2,920\,Byte      \\
		\textit{\tbp IKE SA}									& $\sim$254\,Byte							& $\sim$254\,Byte	\\
		\textit{\tbptwo Client SA}						& $\sim$120\,Byte         		& $\sim$120\,Byte	\\
		\textit{\tbptwo DH SA}								& $\sim$124\,Byte         		& $\sim$124\,Byte	\\
		\hline
		$\sum$ Test Setup (16 Clients)     		& 62,984\,Byte   							& 19,860\,Byte      \\
		\hline
  \end{tabular}
    \centering
    \par\medskip
    \begin{tablenotes}
      \item[a] $2^7*16byte$
			\item[b] $7*16byte$
			\item[c] $2^7*17byte$
			\item[d] $7*17byte$ \\
      \item[e] per client of the group
    \end{tablenotes}
  \end{threeparttable}
\end{table}

==> picture/table-overviewgroupoperations.tex <==

\begin{table*}[t]
%	\footnotesize
	\small
	\centering
	\caption{Summary of the facts}
	\label{tab:overviewgrouoperations}
	\setlength{\tabcolsep}{3pt}
%	\begin{tabular}{llllll}
%         & Send data packets                                            & Encryption   & Notes User & Notes GC & Calculation effort \\ \hline
%\hhline{-----}
%Regist.   & IKE\_SA, $Key_{i}, m_{i}$                                    & 1*A          & 1          & 1*       & normal             \\ \hline
%Intialize & GSA\_AUTH, $CRT(GKEK), XOR_{GKEK}(GTEK)$                     & n*C          & 0/1**      & 1        & normal             \\ \hline
%Join      & GSA\_REKEY(GTEK, GKEK), E(GTEK, GKEK)                        & Re-Key+E     & 0/1**      & 2        & low                \\ \hline
%Leave     & GSA\_REKEY(Tree CRT(GKEK)),  $XOR_{GKEK}(GTEK)$              & 2E ln n/ln 3 & 0/1**      & 1*       & normal             \\ \hline
%Re-Key    & GSA\_REKEY($XOR_{H(GKEK_{Current})}(GKEK_{new}, GTEK_{new})$ & H + XOR      & 0/1**      & 1        & low               \\ \hline

\begin{tabular}{lllllll}
	& Send data packets                                               & Encryption   & Notes User & Notes GC & Keys Length & Effort vs GKMP/SL/LKH \\\hline
	\hhline{-------}
	Regist.   & IKE\_SA, $Key_{i}, m_{i}$                                       & 1$\cdot$A          & 1          & 1*       & 1$\cdot$A + 1$\cdot$E   & normal                \\\hline
	Intialize & GSA\_AUTH, $GKEK_{CRT}, GTEK_{XOR_{GKEK}}$                      & n$\cdot$C          & 0/1**      & 1        & 2$\cdot$E         & normal/low            \\\hline
	Join      & GSA\_REKEY(GTEK, GKEK); $(GTEK, GKEK)_{E}$                      & Re-Key + E     & 0/1**      & 2        & 4$\cdot$E         & low                   \\\hline
	Leave     & GSA\_REKEY($GKEK_{Tree CRT}$),  $GTEK_{XOR_{GKEK}}$             & 2E ln n/ln 3 & 0/1**      & 1*       & 2$\cdot$E         & normal/low            \\\hline
	Re-Key    & GSA\_REKEY($(GKEK_{new}, GTEK_{new})_{XOR_{H(GKEK_{Current})}}$ & H + XOR      & 0/1**      & 1        & 2$\cdot$E         & low                  \\\hline

	\end{tabular}
\end{table*}

%\vspace{-0.6cm}
\begin{table*} [htbp]
	\footnotesize
	\begin{center} 
		\setlength{\tabcolsep}{12pt}
		\begin{tabular}{ll}
n ... Number of group participants &
%L ... Size of the key\\
%G ... Anzahl der Gruppen eines Teilnehmers \hspace*{0.7cm} &
H ... Hashing of a key\\
E ... Symmetric encryption &
A ... Asymmetric encryption\\
C ... Elements included in the CRT/Secure Lock&
k\,\, ... Level of the managed tree\\
* ... Additional effort for key distribution of the tree elements as needed &
** ... Depending on the process initiation (GC/User)\\
		\end{tabular}
	\end{center}
\end{table*}
